Deep Reinforcement Learning, a textbook

Deep reinforcement learning has gathered much attention recently. Impressive results were achieved in activities as diverse as autonomous driving, game playing, molecular recombination, and robotics. In all these fields, computer programs have taught themselves to solve difficult problems. They have learned to fly model helicopters and perform aerobatic manoeuvers such as loops and rolls. In some applications they have even become better than the best humans, such as in Atari, Go, poker and StarCraft. The way in which deep reinforcement learning explores complex environments reminds us of how children learn, by playfully trying out things, getting feedback, and trying again. The computer seems to truly possess aspects of human learning; this goes to the heart of the dream of artificial intelligence. The successes in research have not gone unnoticed by educators, and universities have started to offer courses on the subject. The aim of this book is to provide a comprehensive overview of the field of deep reinforcement learning. The book is written for graduate students of artificial intelligence, and for researchers and practitioners who wish to better understand deep reinforcement learning methods and their challenges. We assume an undergraduate-level of understanding of computer science and artificial intelligence; the programming language of this book is Python. We describe the foundations, the algorithms and the applications of deep reinforcement learning. We cover the established model-free and model-based methods that form the basis of the field. Developments go quickly, and we also cover advanced topics: deep multi-agent reinforcement learning, deep hierarchical reinforcement learning, and deep meta learning.

==> chapters/glos.tex <==
\chapter*{Glossary}





a individual action
R set of rewards
$r_t(s)$ reward at time $t$ of state (s)
V(s) Value function returns the value of a state
Q(s,a) Action-value function, returns the value of action $a$ at
state $s$
$\pi(s)$ Deterministic policy returning the action to take at a state
$\pi(a|s)$ Stochastic policy return the probability that action $a$ is
taken in state $s$
$\pi_\theta$ Policy parameterized by paramaters $\theta$
$\tau$ Trajectory/sequence of states and actions, typically from start
time $t=0$ to end time $t=T$
$G_t$ discounted reward at time $t$
$\mathbb{E}$ Expected value
$\nabla$ Gradient
$\ln$ natural logarithm base $e$
$\theta$ parameters, weights in a deep neural network
$J(\theta)$ Objective function (the goal in reinforcement learning is to
find the policy with the highest cumulative future reward)


%Print list of symbols
\printglossary[type=symbolslist,style=long]


==> chapters/pref.tex <==

{\bf weg? integreren in Introduction?
}


==> chapters/todo.tex <==
\chapter*{To Do}


\begin{enumerate}
\item ml
\item  Basics :: mdp, generalization
\item  Value-based :: model free q, cnn, rnn, overfitting, dqn, rainbow
\item  policy gradients
\item  model based
\item  two agent
\item  multi agent
\item  hierarchical
\item  meta learning
\end{enumerate}


\begin{enumerate}
\item  ml
\item  Tabular RL :: mdp, model free q
\item  Generalization    :: generalization, cnn, rnn, overfitting, dqn, rainbow
\item  policy gradients
\item  model based
\item  two agent
\item  multi agent
\item  hierarchical
\item  meta learning
\end{enumerate}




% Chapter structure:
% \begin{itemize}
% \item unnamed intro
% \item Core problem, concept, algorithms
  
% \item Example: Motivating Achievement
% \item Challenge: PROBLEM
% %\item Application: environment (application to solve)
% \item Approach: AGENT algo challenge and solutions [CORE]
% \item Results: ENVIRONMENT experimental results

% \item exercises
% \item summary
% \end{itemize}

% What kind of book are we?
% A graduate-level textbook

% Do we explain all algorithms? Are we an algorithms cookbook?
% Are we a superficial concepts book?
% Are we in between: 2 (or so) main algos,  in each chapter s=and the rest
% amore superficial treatment.

% \begin{enumerate}
% \item ML, RL
% \item DP-VI, SGD
% \item QL-DQN
% \item REINFORCE-AC-PPO
% \item DynaQ-MPC-ensemble-VPN (integrate Algorithm and Listing) 
% \item Pretraining-MAML  * check algs
% \item MCTS-Selfplay * check algs
% \item CFR-  * check algs
% \end{enumerate}

% Add Thomas Moerland mathematics

% Chapters and Examples
% Examples must be small: enticing teasers to provoke interest. nuggets
% later on at the end of the chapter we present to big, major achievements
% \begin{enumerate}
% \item intro: ML and RL
% \item MDP/Supermarket/Imagenet             DP-DL
% \item Value-Discrete/Maze/Atari            Qlearning-DQN  
% \item Policy-Continuous/Walking/Cheetah    REINFORCE-PPO  
% \item SelfPlay-Given/TD-Gammon/AZ          mcts-az       
% \item Learned/Mountain Car/World-PlaNet     imagination-latent  Google/DeepMind no Schmidhuber
% \item Meta/Pretrain/ZSL                                 
% \item Multi/Negotiation/StarCraft
% \item Summary/Future
% \end{enumerate}
  
  
  

%\begin{itemize}
%  \item first environment, then algorithms. First problem, then solution
  % \item strak eerst environment in elk hoofdstuk zetten. En de rest van
  %   hoofdstuk dan het algoritme opbouwen. 
  %   write in problem/solution style

    % \item waar moet alphazero. in hoofdstuk over model-free? staat hij
    %   nu. bij TD. Dat is raar. In hoofdstuk model-based (planning)
    %   dat is hoofdstuk 2, dat is erg vroeg, en een heel vol hoofdstuk.

      % \item en MCTS staat nu voor DQN, en voor Q-learning, tussen TD
      %   en Q-learning. Dat is raar.
      %   \item of MCTS en AZ moeten in hoofdstuk over learned models
      %     komen. Of apart hoofdstuk, over given models. Wat ze al waren....
% \item 1. do rough placeholder text
% \item reorder story line:
%   \begin{itemize}
%   \item intro chapter
%   \item motivating example
%   \item describe challenges of environment (Question)
%   \item algorithm idea to address those challengess (Answer)
%   \item in-depth algorithm, how it achieved performance
%   \item in-depth environments for further study
%   \item exercises
%   \end{itemize}
% \item use Keras code to describe algorithms like Cherniak?
%   \item use CARDIO as basis (Andrius)?

%   \item 2. rewrite everything to regular nnew text
% \item 3. add exercises and summaries and related work
%   \item split ch6 in given and learned? Allows given to focus on
%     self-play and learned on latent
% \item 4. polish text
% \item 5. polish text again
% \item 6. polish a third time
% \end{itemize}

==> diag/ac.tex <==

\begin{algorithm}[t]
\caption{Actor Critic with bootstrapping and baseline (based on~\cite{sutton2018introduction,weng2018policy})} \label{alg:ac} 
\begin{algorithmic}
\State{{\bf Input:} A differentiable policy $\pi_\theta(a|s)$, $Q_\phi(s,a)$, 
   learning rates $\alpha_\theta, \alpha_\phi \in \mathbb{R}^+$, threshold $\epsilon \in
   \mathbb{R}^+$}
  \State {\bf Initialization}:  Initialize parameters $\theta \in
  \mathbb{R}^d$, $\phi \in \mathbb{R}^d$
  \State Sample $a \sim \pi_\theta(a|s)$
  \Repeat
	\For{$t \in 0,\ldots,T-1$} \Comment{Do for each step of the episode}
 	        \State $r_t \sim  R(s,a)$ \Comment{Sample reward from environment}
                \State $s'\sim T(s'|s,a)$ \Comment{Sample next state
                  from environment}
                \State $a'\sim \pi_\theta(a'|s')$ \Comment{Sample next action}
                \State $A_t=r_t+\gamma^t V_\phi(s')-V_\phi(s)$
                \Comment{Compute Advantage TD error}
                \State $\theta \gets \theta + \alpha_\theta A_t \nabla_\theta\log\pi_\theta(a_t|s_t)$ \Comment{Adjust parameters}
                \State $\phi \gets \phi +
                \alpha_\phi A_t\nabla_\phi V_\phi(s)$
                \Comment{update parameters of action value}
 		\State $a\gets a'$ and $s\gets s'$
	\EndFor
  \Until {$\nabla_\theta J(\theta)$ converges below $\epsilon$}
 \State \Return  Parameters $\theta$
\end{algorithmic}
\end{algorithm}

==> python/pets.tex <==

        \begin{algorithmic}
            \State Initialize policy $\pi_\theta$ and the
            model $\hat{m}_\phi$ \Comment{ensemble}
            \State Initialize an empty dataset $D$
            \For{Trial $k=1, \ldots, K$}
                \State $D\gets$ sample with $\pi_\theta$ from
                environment $E$
                \State Learn one model $ \hat{m}_\phi$ using
                $D$ \Comment probabilistic neural network ensemble
                \For{Time $t=0, \ldots,$ Horizon} \Comment{planning}
                \For{Actions $a_{t:t+T}, \ldots, $NSamples}
                \State Propagate $s$ using Trajectory Sampling and
                $\hat{m}|\{D, a_{t:t+T}\}$ \Comment{ensemble}
                \State Evaluate $r_{t+1}$
                \State Update CEM distribution
                \EndFor
                \State Execute first action $a_t$ from optimal actions
                $a_{t:t+T}$ \Comment{MPC, update $\pi$}
                \State $D\gets D \cup \{s_t, a_t, s_{t+1}\}$
                \EndFor
                \EndFor

        \end{algorithmic}

